A Vocabulary of Board Game Dynamics

In recent years, significant advances have been made in the field of game research. However, there has been a noticeable dearth of scholarly research focused on the domain of dynamics, despite the widespread recognition among researchers of its existence and importance. The objective of this paper is to address this research gap by presenting a vocabulary dedicated to boardgame dynamics. To achieve this goal, we employ a focus group to generate a set of dynamic concepts that are subsequently subjected to validation and refinement through a survey. The resulting concepts are then organized into a vocabulary using a taxonomic structure, allowing the grouping of these concepts into broader and more general ideas.

==> Images/surveyavgSTD.tex <==
\begin{table}
    \centering
        \caption{Averages of answers}
    \begin{tabular}{c|c c|c c}
        Question & Hobbyists & stdev & Professionals & stdev\\
        1 & 4,07 & 1,05 & 4,23 & 0,92\\
        2 & 3,90 & 1,08 & 3,82 & 0,91\\
        3 & 3,92 & 1,11 & 4,36 & 0,73\\
        4 & 4,16 & 1,12 & 4,32 & 0,89\\
        5 & 4,04& 1,14 & 4,50 & 0,74\\
        6 & 3,21& 1,33 & 3,50 & 1,47\\
        7 & 3,35& 1,48 & 3,68 & 1,32\\
        8 & 3,72& 1,21 & 3,73 & 1,08\\
        9 & 2,62& 1,48 & 2,55 & 1,65\\
        10 & 3,48& 1,27 & 3,50 & 1,30\\
        11 & 4,16& 0,98 & 3,86 & 1,28\\
        12 & 3,41& 1,30 & 3,64 & 1,00\\
        13 & 3,17& 1,31 & 3,18 & 1,47\\
        14 & 3,57& 1,19 & 4,05 & 0,90\\
        15 & 3,75& 1,21 & 4,00 & 0,98\\
        16 & 3,01& 1,35 & 3,27 & 1,35\\
        17 & 2,94& 1,47 & 2,55 & 1,53\\
        18 & 4,44& 0,87 & 4,55 & 0,80\\
        19 & 2,68& 1,49 & 2,86 & 1,64\\
        20 & 3,93& 0,99 & 4,00 & 0,98\\
        21 & 3,46& 1,17 & 3,45 & 1,18\\
        22* & 2,88& 1,32 & 3,09 & 1,23\\
        23 & 3,75& 1,28 & 3,68 & 1,21\\
        24 & 3,07& 1,41 & 3,32 & 1,21\\
        25 & 3,78& 1,19 & 4,00 & 1,02\\
        26 & 4,06& 1,02 & 4,32 & 0,65\\
        27 & 4,11& 1,02 & 4,45 & 0,74\\
        28 & 4,34& 0,86 & 4,41 & 0,80\\
        29 & 4,06& 1,00 & 4,14 & 1,13\\
        30* & 2,63& 1,41 & 3,14 & 1,49\\
        31 & 1,88& 1,24 & 2,18 & 1,47\\
        32 & 1,76& 1,19 & 2,09 & 1,54\\ 
        33 & 2,27& 1,36 & 2,50 & 1,60\\
        34 & 3,06& 1,45 & 3,14 & 1,21\\
        35 & 3,71& 1,22 & 4,00 & 1,11\\
        36 & 3,82& 1,04 & 3,82 & 0,96\\
        37* & 2,93& 1,47 & 3,00 & 1,48\\
        38 & 2,07& 1,34 & 2,18 & 1,47\\
        39 & 2,26& 1,26 & 2,27 & 1,45\\
        40 & 3,91& 1,01 & 3,77 & 1,27
    \end{tabular}
    \caption*{* - differences between hobbyists and professionals}
    \caption*{stdev = standard deviation}
    \label{tab:avgResult}
\end{table}
